EquiCity Game: A mathematical serious game for participatory design of spatial configurations

We propose mechanisms for a mathematical social-choice game that is designed to mediate decision-making processes for city planning, urban area redevelopment, and architectural design (massing) of urban housing complexes. The proposed game is effectively a multi-player generative configurator equipped with automated appraisal/scoring mechanisms for revealing the aggregate impact of alternatives; featuring a participatory digital process to support transparent and inclusive decision-making processes in spatial design for ensuring an equitable balance of sustainable development goals. As such, the game effectively empowers a group of decision-makers to reach a fair consensus by mathematically simulating many rounds of trade-offs between their decisions, with different levels of interest or control over various types of investments. Our proposed gamified design process encompasses decision-making about the most idiosyncratic aspects of a site related to its heritage status and cultural significance to the physical aspects such as balancing access to sunlight and the right to sunlight of the neighbours of the site, ensuring coherence of the entire configuration with regards to a network of desired closeness ratings, the satisfaction of a programme of requirements, and intricately balancing individual development goals in conjunction with communal goals and environmental design codes. The game is developed fully based on an algebraic computational process on our own digital twinning platform, using open geospatial data and open-source computational tools such as NumPy. The mathematical process consists of a Markovian design machine for balancing the decisions of actors, a massing configurator equipped with Fuzzy Logic and Multi-Criteria Decision Analysis, algebraic graph-theoretical accessibility evaluators, and automated solar-climatic evaluators using geospatial computational geometry.

==> Paper_Structure.tex <==
%------------------------------------------------------------------------------
%	ALIGHNMENTS
%------------------------------------------------------------------------------

% \usepackage{indentfirst} %indentation of the first paragraph of the section or chapter
\usepackage{microtype}

%------------------------------------------------------------------------------
%	FONTS
%------------------------------------------------------------------------------

\usepackage{times}

%------------------------------------------------------------------------------
%	MATH
%------------------------------------------------------------------------------

\usepackage{fancyhdr,graphicx,amsmath,amssymb, amsfonts,mathtools}
\usepackage{euscript} %euler script
\DeclarePairedDelimiter{\nint}\lfloor\rceil %round to nearest intiger symbol

%------------------------------------------------------------------------------
%	ALGORITHM
%------------------------------------------------------------------------------
%\usepackage{xcolor}
\usepackage[table]{xcolor}% http://ctan.org/pkg/xcolor
%documentation: http://ctan.cs.uu.nl/macros/latex/contrib/xcolor/xcolor.pdf
\usepackage[
	linesnumbered,
	boxed,
	ruled,
	vlined
]{algorithm2e}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}
% algorithm comment style
\newcommand\mycommfont[1]{\scriptsize\ttfamily\textcolor{darkgray}{#1}}
\SetCommentSty{mycommfont}
% algorithm numbering style
\newcommand\mynumfont[1]{\footnotesize\ttfamily\textcolor{darkgray}{#1}}
\SetNlSty{mynumfont}{}{}
% set algorithm caption size
\SetAlCapFnt{\footnotesize}
% set the algorithm font
% \SetAlFnt{\ttfamily}
%\removing the indent of algorithm
\setlength{\algomargin}{1.2em}
% create a while loop construct
\SetKwFor{While}{while}{do}{end}
% for setting the line space in algorithm
\usepackage{setspace}

%------------------------------------------------------------------------------
%	Itemize & Enumerate Options
%------------------------------------------------------------------------------

\usepackage{enumitem}% http://ctan.org/pkg/enumitem
% setting the itemize line spacing for the whole document
\let\OLDitemize\itemize
\renewcommand\itemize{\OLDitemize[noitemsep,topsep=0pt]}
% setting the enumerate line spacing for the whole document
\let\OLDenumerate\enumerate
\renewcommand\enumerate{\OLDenumerate[noitemsep,topsep=0pt]}

%------------------------------------------------------------------------------
%	TABLES, FIGURES & CAPTIONS
%------------------------------------------------------------------------------

\usepackage{multirow,tabularx, booktabs} % advanced table package
\def\arraystretch{1.25} % 25 percent more vertical space for each row
\renewcommand{\tabularxcolumn}[1]{m{#1}} % alighn vertically to the middle

\usepackage[justification=centering, 
font=small, 
labelfont=bf, 
textfont=it]{caption} % package for adding and styling the captions


% placement of floats
\usepackage{float} % to affect the placement of elements
\usepackage{placeins} % to place barriers for float objects
\usepackage{subcaption} % for captioning subfigures

%------------------------------------------------------------------------------
%	BIBLIOGRAPHY
%------------------------------------------------------------------------------

\usepackage{hyperref} % package for refrencing the tables, figures and bibliography
\usepackage[
    backend=biber,
    style=ieee
]{biblatex} % bibliography package and styling

%------------------------------------------------------------------------------
%	CUSTOM FUNCTIONS & MISCELLANEOUS SETTINGS
%------------------------------------------------------------------------------

\newcommand\red[1]{\textcolor{red}{#1}} % red text: texts that needs attention
\newcommand{\comment}[1]{} % multiline comment function

\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}} % new fraction function to prevent the math symbols from getting crammed in a fraction

% \setlength{\emergencystretch}{3em} % relaxing the spacing between letters and words

%------------------------------------------------------------------------------
%	IEEE
%------------------------------------------------------------------------------

% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
% \usepackage{graphicx}
\usepackage{textcomp}
% \usepackage{xcolor}

==> tab/THSD_S.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
Empty DataFrame
Columns: Index(['A', 'B', 'mean(A)', 'mean(B)', 'diff', 'se', 'T', 'p-tukey', 'hedges'], dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}

